Highly Efficient Direct Analytics on Semantic-aware Time Series Data Compression

Semantic communication has emerged as a promising paradigm to tackle the challenges of massive growing data traffic and sustainable data communication. It shifts the focus from data fidelity to goal-oriented or task-oriented semantic transmission. While deep learning-based methods are commonly used for semantic encoding and decoding, they struggle with the sequential nature of time series data and high computation cost, particularly in resource-constrained IoT environments. Data compression plays a crucial role in reducing transmission and storage costs, yet traditional data compression methods fall short of the demands of goal-oriented communication systems. In this paper, we propose a novel method for direct analytics on time series data compressed by the SHRINK compression algorithm. Through experimentation using outlier detection as a case study, we show that our method outperforms baselines running on uncompressed data in multiple cases, with merely 1% difference in the worst case. Additionally, it achieves four times lower runtime on average and accesses approximately 10% of the data volume, which enables edge analytics with limited storage and computation power. These results demonstrate that our approach offers reliable, high-speed outlier detection analytics for diverse IoT applications while extracting semantics from time-series data, achieving high compression, and reducing data transmission.

==> algorithms/semanticQuantization.tex <==
\begin{algorithm}
\caption{Semantic Quantization}
\textbf{Inputs:} $X$ - input data, $\eta$ - SNR \\
\textbf{Output:} $B$ - knowledge base of $X$ \\
\begin{algorithmic}[1]
    \STATE $\epsilon_b \leftarrow$ filter($\eta$)
    \IF{$X'$ cannot be divided}
        \STATE \textbf{return} exNode\{Size $\leftarrow |X'|$\}
    \ELSE
        \STATE let $Q$ be a list of attributes in $X'$
        \STATE randomly select an attribute $q \in Q$
        \STATE randomly select a split point $p$ between the $\text{max}$ and $\text{min}$ values of attribute $q$ in $X'$
        \STATE $X_l \leftarrow \text{filter}(X', q < p)$
        \STATE $X_r \leftarrow \text{filter}(X', q \geq p)$
        \STATE \textbf{return} inNode\{Left $\leftarrow$ iTree($X_l$),
        \STATE \hspace{10mm} Right $\leftarrow$ iTree($X_r$),
        \STATE \hspace{10mm} SplitAtt $\leftarrow q$,
        \STATE \hspace{10mm} SplitValue $\leftarrow p$\}
    \ENDIF
\end{algorithmic}
\label{alg:semanticQuantization}
\end{algorithm}
